Quantitative Measurement of Cyber Resilience: Modeling and Experimentation

Cyber resilience is the ability of a system to resist and recover from a cyber attack, thereby restoring the system's functionality. Effective design and development of a cyber resilient system requires experimental methods and tools for quantitative measuring of cyber resilience. This paper describes an experimental method and test bed for obtaining resilience-relevant data as a system (in our case -- a truck) traverses its route, in repeatable, systematic experiments. We model a truck equipped with an autonomous cyber-defense system and which also includes inherent physical resilience features. When attacked by malware, this ensemble of cyber-physical features (i.e., "bonware") strives to resist and recover from the performance degradation caused by the malware's attack. We propose parsimonious mathematical models to aid in quantifying systems' resilience to cyber attacks. Using the models, we identify quantitative characteristics obtainable from experimental data, and show that these characteristics can serve as useful quantitative measures of cyber resilience.

==> includes/css_and_keywords.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010520.10010553</concept_id>
       <concept_desc>Computer systems organization~Embedded and cyber-physical systems</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010520.10010575.10010577</concept_id>
       <concept_desc>Computer systems organization~Reliability</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
       <concept_id>10002950.10003714.10003727.10003728</concept_id>
       <concept_desc>Mathematics of computing~Ordinary differential equations</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded and cyber-physical systems}
\ccsdesc[500]{Computer systems organization~Reliability}
\ccsdesc[500]{Mathematics of computing~Ordinary differential equations}
\keywords{bonware, cyber resilience, dynamical systems, experimentation,
  malware, mathematical modeling, parameter estimation, quantitative measurement, stability.}


==> includes/obtaining_model_parameters.tex <==
\subsection{Obtaining model parameters}\label{sec:parameters}
Given data that represents functionality over the course of an incident where malware and bonware are active, we develop a fast method to estimate the continuous model parameters for a curve that approximates the data, and use these parameters to generate further realizations based on this model.  In Fig.~\ref{fig:notional}, notional data is shown (in orange) and the parameters $\malware$ and $\bonware$ are estimated and a fit for the functionality $F(t)$ is found that solves the piecewise constant model expressed by Eq.~(\ref{eq:000}). 
In this section, we illustrate our fast method to extract the model parameters from this curve.  %The method was used to determine the coefficients $\malware_i$ and $\bonware_i$ in the piecewise model fit to our experimental data.  For example, in Fig.~\ref{fig:model fits}, a continuous fit to the experimental data is shown, and the parameters $\malware_i$ and $\bonware_i$ are estimated.

The set $P=\{t_0, \hdots, t_K\}$ partitions the scenario timeline, and malware and bonware are constant in each interval $(t_{i-1},t_i), \,\, i=1, \hdots, K. \,\,$  In each interval, $\Qware_i=\malware_i+\bonware_i$ and the differential equation governing Continuous Model I is $\frac{dF(t)}{dt}+\Qware_i F(t) = \Fnominal (t) \bonware_i.$  Thus, in each interval $(t_{i-1},t_i),$ the solution is 
\begin{equation*}
    \functionality(t)     =
    \left(\functionality(t_{i-1}) - \frac{\Fnominal \bonware_i}{
        \Qware_i } \right)  e^{-\Qware_i (t-t_{i-1})} + \frac{\Fnominal \bonware_i}{\Qware_i}.
\end{equation*}
We compute the \impact{} of malware $\malware_i$ and the \impact{} of bonware $\bonware_i$ in each interval.

We observe that there is a unique switching time $\tchange$ where the functionality's trend reverses, and thus we take $K=2.$ Before the switch, the \impact{} of malware is greater than that of bonware. From the time of the switch until the end of the run, bonware is stronger.  To estimate the switching time $\tchange$, we find the minimum of the data to occur over the interval from 64 s to 75 s. There, the minimum value of the data curve is $m=0.27$.  Taking the midpoint, our estimate for $\tchange$ is 69.5 s.

We numerically solve this system of equations:
\begin{align*}
    \alpha m & = \Fnominal \bonQone,                                           \\
    m        & = \left(\functionality(0)  -\Fnominal \bonQone\right) e^{-\Qware_1 \tchange}+\Fnominal \bonQone.                      
\end{align*}
The first equation says that where the curve meets the minimum of the data, it has experienced exponential decay of $\alpha$ toward the asymptotic minimum.  We take $\alpha$ to be $\alpha=1-\sfrac{1}{e}$. The second equation says that the minimum occurs at the switching time (the time when the model switches from malware dominating bonware, to bonware dominating malware).  Solving this system of equations yields (with $\malware_1=\Qware_1-\bonware_1$), $\malware_1 \approx  0.025$ and $\bonware_1 \approx 0.005$.  To the right of $t^\star$, we fit an exponentially increasing function by numerically solving this system of equations:
\newcommand\FBonQtwo[1]{\frac{#1 \bonware_2}{\Qware_2}}
\begin{align*}
    \zeta                & = \FBonQtwo{F(0)},                     \\
    \tilde{\alpha} \zeta & = \left(m- \FBonQtwo{\Fnominal}\right) 
    \!\! \left(e^{-\Qware_2 (125-t^\star)}+\FBonQtwo{\Fnominal}\right).
\end{align*}
We have found that $\tilde{\alpha}=1-e^{-4}$ and $\zeta=0.95$ are satisfactory values to use for these hyperparameters.  We compute $\malware_2 \approx 0.005$ and $\bonware_2 \approx 0.088$.


==> includes/table_one.tex <==
\newcommand{\interval}{(t_j \le t < t_{j+1}), \quad (j=0, \cdots, N-1)}
\newcommand{\headerline}[3]{ #1 & #2 & #3 \\}
\newcommand{\tablelines}[3]{\vspace{3mm} #1  & {\begin{equation*}
      {#2} \end{equation*}}  & \vspace{3mm}  #3\\}

\newcommand\introduced{\ins{Introduced in Section $\star$.
  Applied in Section $\star\star$.}}

  \begin{centering}
    \begin{table*}[htp]
      \caption{Resilience Measures}
      \label{tab:models}
      % \begin{tabular}{ |p{2.25cm}|p{5.75cm}|p{8.75cm}|  }
      \begin{tabular}{ |C{2.00cm}|C{7.75cm}|C{5.75cm}|  }   % see bottom of packages.tex
        \hline
        \headerline{Measure}{Definition}{Notes or Application or Context}
        \hline
        \tablelines{Area Under the Curve}{ \text{AUC}=\frac{1}{T-t_0}
        \int_{t_0}^T F(\tau)\,d\tau }{\introduced {} Illustrated in Figure 1 and in Figures $\cdots$}
        \hline
        \tablelines{Resilience Ratio}{R=\frac{\int_{t_0}^T F_\text{attack}(\tau)\,d\tau}
        {\int_{t_0}^T F_\text{baseline}(\tau)\,d\tau}}{\introduced {} Illustrated in Figures $\cdots$}
        \hline
        \tablelines{Resilience Vector}{{\cal R}=\sum_{j=1}^n u_j R_j, \quad \text{where }
        \sum_{j=1}^n u_j = 1 }{\introduced}
        \hline
        \hline
      \end{tabular}
    \end{table*}
  \end{centering}



==> includes/thank_you.tex <==
\newcommand\thankyou{This work was partially funded by Cyber Technologies,
    Deputy CTO for Critical Technologies/Applied Technology, Office of
    the Under Secretary of Defense Research and Engineering.  Research was sponsored by the Army Research
Laboratory and was accomplished under Cooperative Agreement Number
W911NF-21-2-0284. Dr. Vandekerckhove was additionally supported by NSF \#1850849 and \#2051186.\\ \\
The views and conclusions contained in this document are those of the authors and should not be interpreted as
representing the official policies, either expressed or implied, of
the Army Research Laboratory or the U.S. Government. The
U.S. Government is authorized to reproduce and distribute reprints for
Government purposes notwithstanding any copyright notation herein. }


==> includes/title_and_authors_B0.tex <==
\newcommand\combined{The views and conclusions
  contained in this document are those of the authors and should not
  be interpreted as representing the official policies, either
  expressed or implied, of the Army Research Laboratory or the
  U.S. Government. The U.S. Government is authorized to reproduce and
  distribute reprints for Government purposes notwithstanding any
  copyright notation herein.  This work was partially funded by Cyber
  Technologies, Deputy CTO for Critical Technologies/Applied
  Technology, Office of the Under Secretary of Defense Research and
  Engineering.  Dr.~Vandekerckhove's research was sponsored by the
  Army Research Laboratory Cooperative
  Agreement Number W911NF-21-2-0284 and National Science Foundation grants \#1850849 and \#2051186.}

% \newcommand\devcom{U.S. Army Combat Capabilities Development Command,
%  Army Research Laboratory}
% \newcommand\devcom{US Army Combat Capabilities Development Command, Army Research Laboratory}
% \newcommand\devcom{U. S. Army Combat Capabilities Development Command,
%  Army Research Laboratory}
% \newcommand\devcom{US Army Combat Capabilities Development Command,
% Army Research Laboratory}
\newcommand\devcom{DEVCOM Army Research Laboratory}

\title{Quantitative Measurement of Cyber Resilience: Modeling and Experimentation}

\author{Michael J. Weisman}
% \orcid{0000-0003-4918-5571}
\affiliation{%
            \institution{\devcom}
  \city{Adelphi}
  \state{Maryland}
  \country{USA}
}
\email{michael.j.weisman2.civ@army.mil}

\author{Alexander Kott}
\affiliation{%
         \institution{\devcom}
  \city{Adelphi}
  \state{Maryland}
  \country{USA}
}
\email{alexander.kott1.civ@army.mil}

\author{Jason E. Ellis}
\affiliation{%
        \institution{\devcom}
  \city{Adelphi}
  \state{Maryland}
  \country{USA}
}
\email{jason.e.ellis7.civ@army.mil}

\author{Brian J. Murphy}
\affiliation{%
    \institution{Penn State University}
  \city{State College}
  \state{Pennsylvania}
  \country{USA}
}
\email{bjm206@arl.psu.edu }

\author{Travis W. Parker}
\affiliation{%
    \institution{ICF International}
  \city{Adelphi}
  \state{Maryland}
  \country{USA}
}
\email{travis.w.parker16.ctr@army.mil }

\author{Sidney Smith}
\affiliation{%
    \institution{\devcom}
  \city{Adelphi}
  \state{Maryland}
  \country{USA}
}
\email{sidney.c.smith24.civ@army.mil}

\author{Joachim Vandekerckhove}
\affiliation{%
    \institution{University of California, Irvine}
  \city{Irvine}
  \state{California}
  \country{USA}
}
\email{joachim@uci.edu}

\renewcommand{\shortauthors}{Weisman, et al.}



